Robust stabilization of multiport networks

This paper formulates and solves the problem of robust compensation of multiport active network. This is an important engineering problem as networks designed differ in parameter values due to tolerance during manufacture from their actual realizations in chips and hardware. Parameters also undergo changes due to environmental factors. Hence, practical use of networks requires compensation which is only possible by connecting compensating network at the ports. The resulting interconnection is then required to be stable over a range of parameter values. This is called robust compensation. This paper formulates such a problem using an extension of the coprime factorization theory well known in feedback control theory to the situation of multiport network interconnection developed in \cite{msm1} and formulates the robust stabilization problem as an $H_{\infty}$ optimization problem. The port interconnection of networks does not confirm with computation of the function of the interconnected network analogous to that of the feedback interconnection using signal flow graph. Hence the well known stabilization and stability theory of feedback systems cannot be utilized for such a problem. A new formulation of stabilization theory of network interconnection was formulated and developed by the authors in \cite{msm1}. The variations of parameters of the network are used to define a worst case neighborhood of the network in terms of its coprime fractions at the nominal values of parameters. The solution of the optimization problem is then carried out by the standard procedure of converting such a problem to the Nehari optimization problem \cite{fran}. This methodology of solving the robust compensation of multiport networks using feedback control theory is believed to be novel.

==> garbagedata.tex <==
\chapter{Robust Stabilization }
\section{Introduction}
Active multiport networks always have uncertainties and perturbations because of parameter variations, model errors, disturbances, noise and parasitic effects. The mathematical models for such networks are generally built using the nominal parameter values.
Such a circuit with nominal values may not meet the prescribed performance specifications or even become unstable in actual operating conditions if the robustness aspect is not considered in the compensation design. It is important that the interconnection remain stable even though there is difference between the nominal model and the network under practical conditions.

In this chapter, robust stabilization problem is formulated and solved. Such a problem is well known in systems theory and has well known approaches for its solution \cite{fran, zafr}. The formulation of robust stabilization problem is explained in section \ref{robuststproforsec} while its solution methodology is explained in section \ref{solutionrobuststab}. An illustrative circuit example is shown in \ref{robuststabprobsec} along with results and discussion followed by conclusion in section \ref{robustconsec} 

\section{Formulation of robust stabilization problem}
\label{robuststproforsec}
The stabilization problem in case of multiport networks is already defined in section \ref{multiportstabprob}. Consider a linear time invariant circuit represented by the following equation.
\begin{equation}
\label{multiporteqn}
Y_r  = HU_s
\end{equation}
where $U_s$ denotes the vector of Laplace transforms of the independent sources at the ports and $Y_r$ denotes the vector of Laplace transforms of the responses at the ports (respecting indices). $H$ represents matrix of hybrid network functions between elements of $Y_r$ and $U_s$, respectively and assumed as proper with matrix $D$ in its state space model as non-singular. It has a formal inverse as a proper rational matrix. 

Consider a compensation network of same number and type of independent sources as the given network of (\ref{multiporteqn}) to be compensated at all its port indices. Let a compensating network has a hybrid function matrix $H_{c}$. (As in case of $H$, $H_{c}$ is also assumed to be proper with formal inverse which is proper). Then for the source vector $U_{cs}$ the response vector $Y_{cr}$ in the compensating network is given by the following equation.
\begin{equation}
\label{eqn4}
Y_{cr}= H_c U_{cs}
\end{equation}

The interconnection of ports is said to be in series (respectively parallel) when the common source at the port is a voltage (respectively current) source. If the two multiport networks are connected then the independent source vector, $\hat{U}_{s}$, applied to the interconnection distributes in the two networks as given by the following equation.
%\[
\begin{equation}
\hat{U}_{s}=U_{s}+U_{cs}
\end{equation}
%\]
while the common response vector $\hat{Y}_{r}$ of the two networks at the ports is given by the following equation.
%\[
\begin{equation}
\hat{Y}_{r}=HU_{s}=H_{c}U_{cs}
\end{equation}
%\]
Hence, the source vectors reflected on ports of each network are given by the following equations.
%\[
\begin{equation}
U_{s}=H^{-1}\hat{Y}_{r}, \ \ \ \ \ \mbox{   }U_{cs}=H_{c}^{-1}\hat{Y}_{r}
\end{equation}
%\]
Therefore, for the interconnected network, the source response relationship is given by the following equation.
\begin{equation}\label{TotalResponserelationmult}
\hat{Y}_{r}=(H^{-1}+H_{c}^{-1})^{-1}\hat{U}_{s}
\end{equation}
which is the hybrid representation of the interconnected network. It can be observed that the interconnected network is BSBR stable iff the hybrid matrix of interconnection $(H^{-1}+H_{c}^{-1})^{-1}$ is in $M(\stabS)$. The stabilization problem is defined with additional restriction that the hybrid matrices of the interconnection arising from all $\tilde{H}$, due to uncertainties and perturbations, in a small neighborhood of $H$ are also stable.

This problem can be solved using doubly coprime fractional (DCF) representation explained in the chapter on stabilization and the notion of neighborhood. As stated in theorem \ref {multportstabthm}, there exists a doubly coprime fractions of $H_{c}$ that satisfy the following equation.
\begin{equation}\label{doublycfrelationwithTc}
\left[\begin{array}{rr}
 D_{cl} & N_{cl}\\
 D_{l} & -N_{l} 
\end{array}\right]
\left[\begin{array}{rr}
 N_{r} & N_{cr}\\
 D_{r} & -D_{cr}
\end{array}\right]=
\left[\begin{array}{rr}
 I & 0\\
 0 & I
\end{array}\right]
\end{equation}

Consider $N_{l}$ and $D_{l}$ to be matrices over $M(\stabS)$ at nominal parameter values of a given network. Due to uncertainties, perturbations and model errors, these matrices differ from their nominal values such that $\tilde N_{l}$ and $\tilde {D_{l}}$ form the neighborhood of $N_{l}$ and $D_{l}$. Solving the robust stabilization problem involves finding a compensating network, $H_{c}$ with right coprime fractions $N_{cr},D_{cr}$ such that the interconnection remains stable even in the neighborhood of $N_{l}$ and $D_{l}$.
Let $\Delta$ be the matrix representing the neighborhood of $N_{l}$ and $D_{l}$ and is as given below.
\begin{equation}\Delta = 
\left[\begin{array}{rr}
\tilde N_{l}-N_{l} & \ \ \tilde D_{l}-D_{l}
 \end{array}\right] =
 \left[\begin{array}{rr}
\Delta_{N} & \ \ \Delta_{D}
 \end{array}\right]
\end{equation}
Thus $\tilde N_{l}$ and $\tilde D_{l}$ can be expressed as,
\begin{align}
\tilde N_{l}&=N_{l}+\Delta_{N} \notag \\
\tilde D_{l}&=D_{l}+\Delta_{D}
\end{align} 
Now, consider
\begin{align*}
 \left[\begin{array}{rr}
\tilde N_{l} & \ \ \tilde D_{l}
 \end{array}\right] 
 \left[\begin{array}{rr}
 D_{cr} \\
 N_{cr}
 \end{array}\right] 
 &= 
 \left[\begin{array}{rr}
N_{l}+\Delta_{N} & \ \ D_{l}+\Delta_{D}
 \end{array}\right] 
 \left[\begin{array}{rr}
 D_{cr} \\
 N_{cr}
 \end{array}\right] \\
 &= \Big(
 \left[\begin{array}{rr}
N_{l} & \ \ D_{l}
 \end{array}\right]  
 +
 \left[\begin{array}{rr}
\Delta_{N} & \ \ \Delta_{D}
 \end{array}\right] \Big)
  \left[\begin{array}{rr}
 D_{cr} \\
 N_{cr}
 \end{array}\right]
 \end{align*}
But $N_{l}D_{cr}+D_{l}N_{cr}=I$ and $\Delta =\left[\begin{array}{rr}
\Delta_{N} & \ \ \Delta_{D}
 \end{array}\right]$.
Therefore, the above equation can be simplified as shown below.
\begin{equation}
\left[\begin{array}{rr}
\tilde N_{l} & \ \ \tilde D_{l}
\end{array}\right] 
\left[\begin{array}{rr}
D_{cr} \\
N_{cr}
\end{array}\right] 
=
I + \Delta \left[\begin{array}{rr}
D_{cr} \\
N_{cr}
\end{array}\right] 
\end{equation} 

With nominal parameter values, the identity $N_{l}D_{cr}+D_{l}N_{cr}=I$ is satisfied but with perturbations and disturbances 
$
 I + \Delta \left[\begin{array}{rr}
 D_{cr} \\
 N_{cr}
 \end{array}\right]
 $
 must also belong to $M(\stabS)$ so as to achieve robust stabilization. For this, following equation must be satisfied.
 \begin{equation}
 \Big \Vert \Delta \left[\begin{array}{rr}
 D_{cr} \\
 N_{cr}
 \end{array}\right] \Big \Vert_{\infty}<1
 \end{equation}
 
$\Delta$ represents various matrices based on uncertainties which should satisfy $\Vert \Delta (j\omega)) \Vert \leq R(j\omega) \ \ \forall \ \ \omega \in [0,\infty)$ where $R(j\omega)$ represents the uppermost bound on $\Delta$. In worst case, $\Delta$ can be considered to be equal to $R$ being one of the possible functions. Thus, the robust stabilization problem now reduces to the following. 
\begin{equation}
\Big \Vert R \left[\begin{array}{rr}
D_{cr} \\
N_{cr}
\end{array}\right] \Big \Vert_{\infty}<1
\end{equation}
 
But $D_{cr}$ and $N_{cr}$, from corollary \ref{robustpara1} in section \ref{multiportstabprob}, are respectively given as $(X_{r}-D_{r}Q)$ and $(Y_{r}+N_{r}Q)$ in terms of a free parameter matrix $Q$. Thus, the robust stabilization problem can further be simplified as below.
 \begin{equation}
 \label{robuststabi1}
 \Big \Vert R \left[\begin{array}{rr}
X_{r}-D_{r}Q \\
Y_{r}+N_{r}Q
 \end{array}\right] \Big \Vert_{\infty}<1
 \end{equation}
Simplifying equation (\ref{robuststabi1}) further gives,
\begin{equation}
\label{robuststabfor}
\Big \Vert R 
\left[\begin{array}{rr}
X_{r} \\
Y_{r}
\end{array}\right] - R
\left[\begin{array}{rr}
D_{r} \\
-N_{r}
\end{array}\right] Q \Big \Vert_{\infty}<1 
\equiv
\Vert T_{1}-T_{2}Q\Vert_{\infty}<1
\end{equation}
Hence, the robust stabilization problem can be solved iff there a solution to the following optimization problem,
\beq
\min_{Q\in M(\stabS)} \Vert T_{1}-T_{2}Q\Vert_{\infty}<1
\eeq
This formulation of the robust stabilization problem is mathematically identical to the well known formulation in feedback control theory and also has well known approaches for solution \cite{fran}.

\section{Solution to robust stabilization problem}
\label{solutionrobuststab}
The solution to robust stabilization problem is explored in this section. Here, $T_{i}$' s are matrix valued functions. The problem is lot harder to solve as compared to when they are scalar valued. This problem is typically a model matching problem which computes a matrix $Q$ in $\stabS$ so as to minimize $\Vert T_{1}-T_{2}Q\Vert$ from known matrices $T_{1}$ and $T_{2}$. \\
Let $\gamma$ denote the infimal model matching error as given below.
\begin{equation}
\gamma := \textrm{inf}\{\Vert T_{1}-T_{2}Q\Vert_{\infty} : Q \in \stabS \}
\end{equation} 
It can be solved by computing the upper bound $\beta$ for $\gamma$ such that $\beta-\gamma$ is less than a pre-specified tolerance and then $Q$ in $\stabS$ can be computed which satisfies the given robust stabilization problem as below.
\beq
\min_{Q\in M(\stabS)} \Vert T_{1}-T_{2}Q\Vert_{\infty}\leq \beta
\eeq
$Q$ obtained after solving this problem may not be optimal but it will be as near optimality as desired.

For solving such a problem in scalar case, one of the approaches as described in \cite{fran}, is to reduce it to a Nehari problem which approximates $RL_{\infty}$ matrix\footnote{A $RL_{\infty}$ matrix is a real rational matrix which is proper and has no poles on imaginary axis.} by a matrix belonging to $\stabS$. The problem can be simplified by bringing in an inner-outer factorization of $T_{2}$ as $T_{2}=T_{2i}T_{2o}$. For $Q$ in $\stabS$, following simplification can be carried out.  
\begin{align*}
\Vert T_{1}-T_{2}Q\Vert &= \Vert T_{1}-T_{2i}T_{2o}Q\Vert  \\
&=\Vert T_{2i}(T_{2i}^{-1} T_{1}-T_{2o}Q\Vert  \\ 
&=\Vert T_{2i}^{-1}T_{1}-T_{2o}Q\Vert  \\ 
&=\Vert R-X \Vert
\end{align*}

This simplification is possible due to the property of the inner factor $\vert T_{2i}(j\omega)\vert=1$. The inner factor does not affect the infinity norm and can be taken out from the norm.    

The Nehari problem can be posed as:- Given $R$ in $RL_{\infty}$ with dist $(R,\stabS)<1$, find all $X's$ in $\stabS$ such that   $\Vert R-X \Vert_{\infty}\leq 1$. Only some of these are closest to $R$ that satisfy  
$\Vert R-X \Vert_{\infty}=$ dist$(R,\stabS)$.

It is required to find the distance from an $L_{\infty}$ matrix $R$ to $\stabS$. In systemic terms, a given unstable transfer function in $L_{\infty}$ norm is to be approximated by a stable one. Nehari's theorem is an elegant solution to this problem. A lower bound for the distance can be easily obtained. Fix $X$ in $\stabS$ then $\Vert R-X \Vert_{\infty}= \Vert \Gamma_{R}\Vert $ where $\Gamma_{R}$ is the Hankel operator. $ \Vert \Gamma_{R}\Vert $ is a lower bound for the distance $R$ to $\stabS$. Nehari's theorem states that there exists a closest matrix $X$ in $\stabS$ to a given matrix $R$ in $L_{\infty}$ and $\Vert R-X \Vert =\Vert \Gamma_{R}\Vert$. 

In general, there are many $X$'s nearest $R$. The time domain interpretation of Nehari's theorem states that the distance from a given noncausal system to the nearest causal linear and time invariant one equals the norm of the Hankel operator. Alternatively, the norm of the Hankel operator is a measure of non-causality.

To see the systematic development for the solution to robust stabilization problem in matrix case, first an inner-outer factorization of $T_{2}$ can be carried out as $T_{2}=U_{i}U_{o}$ where $U_{i}$ is inner and $U_{o}$ is outer. Define $RL_{\infty}$ matrix $Y$ as $Y:=I-U_{i}U_{i}^{*}T_{1}$ where $U_{i}^{*}$ is complex conjugate transpose of the matrix $U_{i}$. For defining the spectral factorization of a matrix, consider a square matrix $G(s)$ which satisfies the following properties. 
\begin{align}
G,G^{-1} \ &\in RL_{\infty} \notag \\
G^{*} &= G \notag \\
G(\infty) &>0 \notag 
\end{align}
Such a matrix has pole and zero symmetry about the imaginary axis. $G$ can be factored as $G=G_{-}^{*} G$ where $G_{-},G_{-}^{-1} \in \stabS$. This is called a spectral factorization of $G$ and $G_{-}$ is a spectral factor.  

If $\beta$ is a real number greater than $\Vert Y \Vert_{\infty}$, then the matrix $\beta^{2}-Y^{*}Y$ has a spectral factor $Y_{o}$ where $Y^{*}$ is complex conjugate transpose of the matrix $Y$. Let $R$ be defined as a 
$RL_{\infty}$ matrix as $R:=U_{i}^{*}T_{1}Y_{o}^{-1}$. Thus, $R$ depends on $\beta$. It is now required to find a closest matrix $X$ in $\stabS$ to a given matrix $R$ in $L_{\infty}$.

Following are the two preliminary technical facts that need to be considered before stating the main theorem for finding $X$ in $\stabS$ in the form of lemmas as found in \cite {fran} without proofs and used in the derivation of the main theorem.
\begin{lem}\label{lema1}\emph{
If $U$ is an inner matrix and $E$ is an $RL_{\infty}$ matrix 
\begin{equation*}
 E:= \Big \Vert  \left[\begin{array}{rr}
 U^{*} \\
 I-UU^{*}
 \end{array}\right] \Big \Vert_{\infty}
 \end{equation*}
then $\Vert EG \Vert_{\infty}=\Vert G \Vert_{\infty} $ for all matrices $G$ in $RL_{\infty}$ matrix.}
\end{lem}
\begin{lem}\label{lema2}\emph{
If $F$ and $G$ are $RL_{\infty}$ matrices with equal number of columns and if
\begin{equation*}
 \Big \Vert  \left[\begin{array}{rr}
 F \\
 G
 \end{array}\right] \Big \Vert_{\infty} < \beta
 \end{equation*}
then $\Vert G \Vert_{\infty} < \beta$ and $\Vert FG_{o}^{-1} \Vert_{\infty} < 1$ where $G_{o}$ is a spectral factor of $\beta^{2}-G^{*}G$.  Conversely, if $\Vert G \Vert_{\infty} < \beta$ holds and $\Vert FG_{o}^{-1} \Vert_{\infty} < 1$, then 
\begin{equation*}
 \Big \Vert  \left[\begin{array}{rr}
 F \\
 G
 \end{array}\right] \Big \Vert_{\infty} \leq \beta
 \end{equation*}
}
\end{lem}

With these preliminary results, the main theorem can now be stated which gives $X$ in $\stabS$ such that $\Vert R-X \Vert_{\infty}<1$ from which $Q$ in $\stabS$ can be obtained. The proof for the theorem as given in \cite{fran} indicates the approach for finding the solution to robust stabilization problem.

\begin{theorem}
\begin{enumerate}
    \item $\gamma := \textnormal{inf}\{\beta: \Vert Y \Vert_{\infty} < \beta, \ \textnormal{dist}(R,\stabS)<1\}$
    \item \textnormal{Suppose} $\beta > \gamma,\ Q,X \in \stabS$,\ $\Vert R-X \Vert_{\infty}\leq 1$ \textnormal{and} $X=U_{o}QY_{o}^{-1}$
\end{enumerate}
\textnormal{Then} $\Vert T_{1}-T_{2}Q\Vert_{\infty} \leq \beta $
\end{theorem}

\begin{proof}
Part ($1$) of this theorem provides a method for computing an upper bound $\beta$ for $\gamma$ while part ($2$) yields a procedure for computation of a nearly optimal $Q$.

Let $\beta_{inf} := \textnormal{inf}\{\beta: \Vert Y \Vert_{\infty} < \beta, \ \textnormal{dist}(R,\stabS)<1\}$.
Choose $\epsilon>0$ and then choose $\beta$ such that $\gamma + \epsilon > \beta > \gamma$. Then, there exists $Q$ in $\stabS$ such that $\Vert T_{1}-T_{2}Q\Vert_{\infty} \leq \beta$.
From lemma \ref{lema1},
\begin{align*}
 \Big \Vert  \left[\begin{array}{rr}
 U_{i}^{*} \\
 I-U_{i}U_{i}^{*}
 \end{array}\right] (T_{1}-T_{2}Q)\Big \Vert &< \beta \\
 \Big \Vert  \left[\begin{array}{rr}
 U_{i}^{*} \\
 I-U_{i}U_{i}^{*}
 \end{array}\right] T_{1} -
 \left[\begin{array}{rr}
 U_{i}^{*} \\
 I-U_{i}U_{i}^{*}
 \end{array}\right] 
 T_{2}Q \Big \Vert &< \beta
 \end{align*}
Now, consider
\begin{equation*}
 \left[\begin{array}{rr}
 U_{i}^{*} \\
 I-U_{i}U_{i}^{*}
 \end{array}\right] 
 T_{2}=  
 \left[\begin{array}{rr}
 U_{i}^{*} \\
 I-U_{i}U_{i}^{*}
 \end{array}\right] 
 U_{i}U_{o} =
 \left[\begin{array}{rr}
 U_{o} \\
 0
 \end{array}\right] 
  \end{equation*}
 Therefore, 
 \begin{align*}
 \Big \Vert  \left[\begin{array}{rr}
 U_{i}^{*} \\
 I-U_{i}U_{i}^{*}
 \end{array}\right] T_{1} -
 \left[\begin{array}{rr}
 U_{o} \\
 0
 \end{array}\right] Q
 \Big \Vert_{\infty} &< \beta \\
 \therefore \Big \Vert  \left[\begin{array}{rr}
 U_{i}^{*}T_{1}-U_{o}Q \\
 (I-U_{i}U_{i}^{*})T_{1}
 \end{array}\right] 
 \Big \Vert_{\infty} &< \beta \\
 \therefore \Big \Vert  \left[\begin{array}{rr}
 U_{i}^{*}T_{1}-U_{o}Q \\
 Y
 \end{array}\right] 
 \Big \Vert _{\infty} &< \beta
 \end{align*} 
 From lemma (\ref{lema2}), 
 \begin{align}
 \Vert Y \Vert_{\infty} & < \beta \\
 \label{spectfactineq}
 \Vert U_{i}^{*}T_{1}Y_{o}^{-1}-U_{o}QY_{o}^{-1} \Vert_{\infty} & < 1
 \end{align}
 
Inequality (\ref{spectfactineq}) implies dist $(R,\ U_{o} \ \stabS  Y_{o}^{-1})<1$. But, $U_{o}$ is right invertible in $\stabS$ and $Y_{o}$ is invertible in $\stabS$. Therefore, $U_{o} \ \stabS  Y_{o}^{-1} = \stabS$ and hence dist $(R,\stabS) <1$. 

From $\Vert Y \Vert_{\infty} < \beta$, dist $(R,\stabS) <1$ and definition of $\beta_{inf}$, it can be concluded that $\beta_{inf} \leq \beta$. Thus, $\beta_{inf} < \gamma+\epsilon$. Since $\epsilon$ is arbitrary, $\beta_{inf} \leq \gamma$.   
 
Now for the reverse inequality, select $\epsilon>0$ and then choose $\beta$ such that $\beta_{inf}+\epsilon>\beta>\beta_{inf}$. Then, $\Vert Y \Vert_{\infty} < \beta$, dist $(R,\stabS) <1$ hold. So, $\Vert U_{i}^{*}T_{1}Y_{o}^{-1}-U_{o}QY_{o}^{-1} \Vert_{\infty}<1$ also holds for some $Q$ in $\stabS$. From lemma (\ref{lema2}),
 \begin{align*}
 \Big \Vert  \left[\begin{array}{rr}
 U_{i}^{*}T_{1}-U_{o}Q \\
 Y
 \end{array}\right] 
 \Big \Vert _{\infty} \leq \beta
 \end{align*} 
 This results in $\Vert T_{1}-T_{2}Q\Vert_{\infty} \leq \beta$. Therefore, $\gamma \leq \beta < \beta_{inf}$ so $\gamma \leq \beta_{inf}$.
 \end{proof}
 
It is required to find $X$ such that $\Vert R-X\Vert_{\infty} \leq 1$ which gives $Q$ such that $\Vert T_{1}-T_{2}Q\Vert_{\infty} \leq \beta$ and the optimization problem is solved. The algorithm as found in \cite{fran} for computing nearly optimal $Q$ is as given below.
\begin{enumerate}
\item [\textbf {Step 1}] Compute $Y$ and  $\Vert Y \Vert_{\infty}$ where $Y:=(I-U_{i}U_{i}^{*})T_{1}$. $U_{i}$ is the inner factor of $T_{2}$ 
\item [\textbf {Step 2}] Find an upper bound $\gamma_{1}$ for $\gamma$. The simplest bound is $\gamma_{1}=\Vert T_{1}
\Vert_{\infty}$.
\item [\textbf {Step 3}] Select a trial value for $\beta$ in the interval ($\Vert Y \Vert_{\infty}, \gamma_{1}$). Binary search can be used to iterate on $\beta$.
\item [\textbf {Step 4}] Compute $R$ and $\Vert \Gamma_{R} \Vert$. Then $\Vert \Gamma_{R} \Vert < 1$ iff $\gamma < \beta$. Increase or decrease the value of $\beta$ accordingly and return to \textbf {Step 3}. With a sufficiently accurate upper bound for $\gamma$ is obtained, continue to \textbf {Step 5}.
\item [\textbf {Step 5}] Find a matrix $X$ in $\stabS$ such that $\Vert R-X \Vert_{\infty}\leq 1$.
\item [\textbf {Step 6}] Solve for $Q$ in $\stabS$ as $X=U_{o}QY_{o}^{-1}$. It is easier to solve this equation for $Q$ if $U_{o}$ is square than when it is not square.   
\end{enumerate}
The illustrative example solved in the next section shows the design of a compensator for a given network such that the interconnected network is robustly stable under parametric variations.

\section{Illustrative example for robust stabilization problem}
\label{robuststabprobsec}
In this section, an illustrative example is solved to show the design of a robust compensator for a given network in order to achieve the robust stability under parametric variations. To obtain such a compensating network, it is required to solve the robust stabilization problem as posed in section \ref{solutionrobuststab}. 

Consider the single port network as shown in the Fig.\ref{fig03:name} excited by a current source. The impedance for this network can be found using Kirchhoff's laws. 
\begin{figure}[!ht]
\centering
\includegraphics[width=9cm,height=4cm]{sensminfig2}
\caption{Single port network example for robust stabilization }\label{fig03:name}
\end{figure}
Applying KCL at node 1,
\begin{equation}
\label{keqn1}
i=\frac{v}{R_{1}}+\frac{v-v_{1}}{sL_{1}}=\frac{v}{R_{1}}+\frac{v}{sL_{1}}-\frac{v_{1}}{sL_{1}}=\Big(\frac{1}{R_{1}}+\frac{1}{sL_{1}}\Big)v-\Big(\frac{1}{sL_{1}}\Big)v_{1}
\end{equation}
Applying KCL at node 2,
\begin{align}
\label{keqn2}
\frac{v-v_{1}}{sL_{1}}&=\frac{v_{1}}{\Big(\frac{1}{sC_{1}}\Big)}+2i_{1}+\frac{v_{1}}{sL_{2}+R_{2}} \notag \\
&= sC_{1}v_{1} + 2\Big(\frac{v-v_{1}}{sL_{1}}\Big)+\frac{v_{1}}{sL_{2}+R_{2}} \notag \\
%&=\Big(s+\frac{1}{s+3}\Big)v_{1}+2i_{1}\notag \\
\therefore -\frac{v-v_{1}}{sL_{1}}&=\Big(sC_{1}+\frac{1}{sL_{2}+R_{2}}\Big)v_{1}\notag \\
\therefore -\frac{v}{sL_{1}}&=\Big(sC_{1}+\frac{1}{sL_{2}+R_{2}}-\frac{1}{sL_{1}}\Big)v_{1} \notag \\
\therefore v_{1}&=\Big[\frac{-(sL_{2}+R_{2})}{L_{1}L_{2}C_{1}s^{3}+L_{1}C_{1}R_{2}s^{2}+(L_{1}-L_{2})s-R_{2}}\Big]v 
\end{align}
%But $i_{1}=\Big(\frac{v-v_{1}}{2s}\Big)$. Substituting for $i_{1}$ in equation (\ref{keqn2}) we get $Z(s)$ given by following equation.
%\begin{align}
%\label{keqn3}
%\Big(\frac{v-v_{1}}{2s}\Big)-2\Big(\frac{v-v_{1}}{2s}\Big) &= \Big(\frac{s^{2}+3s+1}{s+3}\Big)v_{1} \notag\\
%\Longrightarrow  -\Big(\frac{v-v_{1}}{2s}\Big)=\Big(\frac{s^{2}+3s+1}{s+3}\Big)v_{1} \notag\\
%\therefore -\Big(\frac{v}{2s}\Big)&=\Big[\frac{2s^3+6s^2+s-3}{2s(s+3)}\Big]v_{1} \notag \\
%\therefore v_{1}&=\Big[\frac{-(s+3)}{2s^3+6s^2+s-3}\Big]v
%\end{align}
Substituting $v_{1}$ obtained in terms of $v$ from equation (\ref{keqn2}) in equation (\ref{keqn1}), following equation can be obtained.
\begin{align}
\label{kequn3}
i&=\Big(\frac{1}{R_{1}}+\frac{1}{sL_{1}}\Big)v-\Big(\frac{1}{sL_{1}}\Big)\Big[\frac{-(sL_{2}+R_{2})}{L_{1}L_{2}C_{1}s^{3}+L_{1}C_{1}R_{2}s^{2}+(L_{1}-L_{2})s-R_{2}}\Big]v  \notag \\
\therefore i&= \Big[\frac{sL_{1}+R_{1}}{sL_{1}R_{1}}+\frac{sL_{2}+R_{2}}{sL_{1}(L_{1}L_{2}C_{1}s^{3}+L_{1}C_{1}R_{2}s^{2}+(L_{1}-L_{2})s-R_{2})}\Big]v 
\end{align}
The admittance $Y$, of the single port network after simplifying equation (\ref{kequn3}), is as given below.
\begin{align}
\label{kequn4}
Y(s)&=\frac{I(s)}{V(s)}=\frac{L_{1}L_{2}C_{1}s^3+(L_{1}C_{1}R_{2}+L_{2}C_{1}R_{1})s^2+(L_{1}-L_{2}+C_{1}R_{1}R_{2})s+(R_{1}-R_{2})}{R_{1}L_{1}L_{2}C_{1}s^3+R_{1}R_{2}L_{1}C_{1}s^2+R_{1}(L_{1}-L_{2})s-R_{1}R_{2}}  
\end{align}
The impedance $Z$, of the single port network can be obtained by taking the reciprocal of the equation (\ref{kequn4}) which is as given below.  
\begin{align}
Z(s)&=\frac{V(s)}{I(s)}=\frac{R_{1}L_{1}L_{2}C_{1}s^3+R_{1}R_{2}L_{1}C_{1}s^2+R_{1}(L_{1}-L_{2})s-R_{1}R_{2}}{L_{1}L_{2}C_{1}s^3+(L_{1}C_{1}R_{2}+L_{2}C_{1}R_{1})s^2+(L_{1}-L_{2}+C_{1}R_{1}R_{2})s+(R_{1}-R_{2})}
\end{align}
At nominal parameter values $R_{1}=1 \Omega, R_{2}=3 \Omega, L_{1}=2H, L_{2}=1H $ and $C_{1}=1F$, following are the expressions for $Z(s)$ and $Y(s)$.
\begin{align}
Y(s)&=\frac{2s^{3}+7s^2+4s-2}{2s^{3}+6s^2+s-3}=\frac{(s+2.5707)(s+1.2424)(s-0.3131)}{(s+2.5811)(s+1)(s-0.5811)} \\
Z(s)&=\frac{2s^{3}+6s^2+s-3}{2s^{3}+7s^2+4s-2}=\frac{(s+2.5811)(s+1)(s-0.5811)}{(s+2.5707)(s+1.2424)(s-0.3131)}
%&=\frac{s^2+0.9293s-0.389}{s^2+0.4189s-0.5811}
\end{align}

The pole-zero plot of $Z(s)$ at nominal parameter values is as shown in the Fig.\ref{fig06b:name}. The left half plane pole (zero) of $Y(s)$ ($Z(s)$) at $s=-2.5811$ and zero (pole) of $Y(s)$ ($Z(s)$) at $s=-2.5707$ are located approximately at the same location. Hence, they can be cancelled so as to obtain the minimal realization for $Y(s)$ and $Z(s)$) which are, respectively given by the following equations. 
\begin{figure}[h]
\centering
\includegraphics[width=15.0cm,height=10cm]{polezeroz}
\caption{Pole-zero plot of $Z$}\label{fig06b:name}
\end{figure}
\begin{align}
Y(s)&=\frac{s^2+0.9293s-0.389}{s^2+0.4189s-0.5811}=\frac{(s+1.2424)(s-0.3131)}{(s+1)(s-0.5811)} \\
\label{impedance}
Z(s)&=\frac{s^2+0.4189s-0.5811}{s^2+0.9293s-0.389}=\frac{(s+1)(s-0.5811)}{(s+1.2424)(s-0.3131)}
%&=\frac{s^2+0.9293s-0.389}{s^2+0.4189s-0.5811}
\end{align}
A model of the compensating network shall be determined which under parametric variations of the given network ensures the stability of the interconnected network.
%source series connection at the port will ensure the stability and reduce sensitivity of the voltage at the port below a desired frequency domain profile.

The given one port network at nominal parameter values is neither open circuit stable as the pole at $s=0.3131$ of its impedance function $Z(s)$ lies in open RHP nor short circuit stable as the pole at $s=0.5811$ of its admittance function $Y(s)$ lies in open RHP. A compensating network can be designed so as to make the resultant network open circuit stable under the variations in parameters. For this, consider that $\pm 5\%$ variations occur in the parameters of the given single port network.  

The stabilizing compensator $Y_{c}=Z_{c}^{-1}$ is a parallel admittance and set of all such stabilizing $Z_{c}$ has parametrization as $Z_{c}=(Y+QN)(X-QD)^{-1}$ where $Q$ is an arbitrary element of $\stabS$ such that $X-QD\neq0$. It is required to find $Q$ such that the interconnected network is robustally stable under parametric variations.

In this case, the port relation is $V=ZI$. Hence, $H=Z$, $H^{-1}=Y=1/Z$. $H$ is represented by coprime fractions, $Z=ND^{-1}$ where $N,D$ are in $\stabS$. Using the coprime factors,$N, D$ of $Z$, it is possible to obtain two rational functions $X$ and $Y$ such that $NX+DY=1$ holds. The source series compensation is provided by an admittance $Y_{c}=1/Z_{c}$ connected in parallel with $Y$. %as shown in figure \ref{fig00:name}. 
Such a compensator has coprime representation $Z_{c}=N_{c}D_{c}^{-1}$. \\ 
The coprime fractions $N$ and $D$ for $Z$ as given by equation (\ref{impedance}) at nominal parameter values are as below.
\begin{align}
N(s)&=
\frac{s^{2}+0.4189s-0.5811}{s^{2}+3s+2} = \frac{s-0.5811}{s+2} \\
D(s)&=\frac{s^2+0.9293s-0.389}{s^2+3s+2}=
\frac{(s+1.2424)(s-0.3131)}{(s+1)(s+2)}
\end{align}
The solutions to Bezout's identity $XN+YD=1$ give $Y(s)$ and $X(s)$ as below.
\begin{align}
X(s)&=
\frac{-16.9s-20.92}{s^{2}+3s+2} \\
Y(s)&=
\frac{s+20.97}{s+2}
\end{align}

The solution to robust stabilization problem involves finding $R(j\omega)$ which represents an uppermost bound on uncertainties represented by $\Delta$. To find this uppermost bound, it is required to consider the network functions with parametric variations.  Consider $\pm 5\%$ variations occur in the parameters of this network. For each set of variations, $\tilde Z$ and its respective coprime fractions $\tilde N$ and $\tilde D$ needs to be computed. With $N$ and $D$ as coprime fractions at nominal parameter values and $\tilde N$ and $\tilde D$ as coprime fractions at each set of parameter variations, following matrix can be formed.   
\begin{equation}
\label{perturbmatrix}
\left[\begin{array}{rr}
\tilde N-N\\
\tilde D-D  
\end{array}\right]
\end{equation}

There are five parameters and each of these parameters can take $+5\%$ and $-5\%$ apart from its nominal value. Thus, each of these parameters undergoes three possible states ($-5\%$, nominal value and $+5\%$) which forms $3^{5}=243$ possible combinations of the perturbed network impedances and corresponding coprime fractions for each need to be computed.

In order to obtain the uppermost bound, it is required to compute $\infty$ norm of each matrix as given by the equation (\ref{perturbmatrix}) where $\tilde N$ represents the coprime fraction of the perturbed network impedance for each of the parameter variations while $N$ represents the coprime fraction of the network impedance with nominal parameter values. Thus, $3^{5}-1=243-1=242$ matrices are required to be considered for computing the $\infty$ norm at various frequency points wherein the robust stabilization problem needs to be solved. Calculations for one of the variations in the parameters out of different possible combinations of parametric variations is shown here as an illustration.\\
In the network function $Z$, let each of the parameter is undergoing a variation of say $+5\%$ from its nominal value so that  $\tilde R_{1}=1.05 \Omega, \tilde R_{2}=3.15 \Omega, \tilde L_{1}=2.1H, \tilde L_{2}=1.05H $ and $\tilde C_{1}=1.05F$, following expression for perturbed impedance, $\tilde Z(s)$ is obtained.
\begin{align}
\tilde Z&=\frac{2.4310s^{3}+7.2930s^2+1.1025s-3.3075}{2.3152s^{3}+8.1033s^2+4.5228s-2.1} =\frac{1.05(s+2.631)(s+0.9268)(s-0.5579)}{(s+2.624)(s+1.171)(s-0.2951)} \notag \\ 
\label{tildeimpedance}
\therefore \tilde Z&=\frac{1.05(s+0.9268)(s-0.5579)}{(s+1.171)(s-0.2951)}
\end{align} \\
The coprime fractions $\tilde N$ and $\tilde D$ for $\tilde Z$ as given by equation (\ref{tildeimpedance}) for $+5\%$ parameter variation are as below.
\begin{align}
\tilde N &=
\frac{1.05s^{2}+0.3874s-0.543}{s^{2}+3s+2} = \frac{1.05(s+0.9268)(s-0.5579)}{(s+1)(s+2)} \\
\tilde D &=\frac{s^{2}+0.8759s-0.3456}{s^{2}+3s+2}=
\frac{(s+1.171)(s-0.2951)}{(s+1)(s+2)}
\end{align}
The solutions to Bezout's identity $\tilde X \tilde N+\tilde Y \tilde D=1$ give $\tilde Y$ and $\tilde X$ as below.
\begin{align}
\tilde X&=
\frac{-17.9s-20.92}{s^{2}+3s+2} = \frac{-17.9(s+1.1687)}{(s+1)(s+2)}\\
\tilde Y&=\frac{s^{2}+23.92s+21.29}{s^{2}+3s+2}=\frac{(s+22.99)(s+0.9259)}{(s+1)(s+2)}
\end{align}
Thus, following equations are obtained.
\begin{align}
\tilde N-N &=\frac{0.05(s^{2}-0.632s+0.765)}{(s+1)(s+2)}\\
\tilde D-D&=\frac{-0.053s+0.0433}{s^{2}+3s+2}=\frac{-0.05343(s-0.817)}{(s+1)(s+2)}
\end{align}
Using above equations, following matrix can be obtained.
\begin{equation}
\label{perturbmatrixexample}
\left[\begin{array}{rr}
\tilde N-N\\
 \tilde D-D  
\end{array}\right]=
\left[\begin{array}{rr}
\frac{0.05(s^{2}-0.632s+0.765)}{(s+1)(s+2)}\\ \\
\frac{-0.05343(s-0.817)}{(s+1)(s+2)}
\end{array}\right]
\end{equation}

In the matrix given by equation (\ref{perturbmatrixexample}), various frequencies over which robust stabilization problem is required to be solved can be substituted and at each frequency, infinity norm of the matrix can be computed. The variation of this infinity norm with frequency can then be plotted. 

For each of the parameter variations, it is required to compute first the matrix as given by equation (\ref {perturbmatrix}) and then its infinity norm for various frequency points. The variation of this infinity norm with frequency for each of the matrix can then be plotted. Such a plot is as shown in the Fig.\ref{fig05:name}.
\begin{figure}[!ht]
\centering
\includegraphics[width=15.8cm,height=9cm]{rfunction1}
\caption{Variation of infinity norms of perturbed matrices (absolute value) with frequencies}\label{fig05:name}
\end{figure} 
The same plot with db values plotted on Y-axis is as shown in the Fig.\ref{fig06:name}.
\begin{figure}[!ht]
\centering
\includegraphics[width=16.2cm,height=9.4cm]{rfunction1db}
\caption{Variation of infinity norms of perturbed matrices (in db) with frequencies}\label{fig06:name}
\end{figure} 
From the family of loci, the uppermost bound $R(j\omega)$ can be computed.

All the other functions will lie below this uppermost bound. Such a function $R(s)$ can be found and is given by the following equation with its Bode magnitude plot as shown in the Fig.\ref{fig06b:name}.
\begin{equation}
R(s)=\frac{0.06(s+6)}{s+3.4}    %substitute actual function
\end{equation} 
\begin{figure}[!ht]
\centering
\includegraphics[width=16.2cm,height=9.4cm]{magplotws}
\caption{Bode magnitude plot of $R(s)$}\label{fig06b:name}
\end{figure} \\
As seen from equation (\ref{robuststabfor}),
\begin{equation}\label{robuststabequnpara1}
T_{1}=R
\left[\begin{array}{rr}
 X_{r}\\
 Y_{r}  
\end{array}\right]=\frac{0.06(s+6)}{s+3.4}
\left[\begin{array}{rr}
\frac{-16.9s-20.92}{s^{2}+3s+2}\\
\frac{s+20.97}{s+2}  
\end{array}\right]=\left[\begin{array}{rr}
\frac{-1.014(s+1.238)(s+6)}{(s+1)(s+2)(s+3.4)}\\
\frac{0.06(s+20.97)(s+6)}{(s+2)(s+3.4)}  
\end{array}\right]
\end{equation}
\begin{equation}\label{robuststabequnpara2}
T_{2}=R
\left[\begin{array}{rr}
 D_{r}\\
 -N_{r}  
\end{array}\right]=
\left[\begin{array}{rr}
\frac{0.06(s+1.242)(s+6)(s-0.3131)}{(s+1)(s+2)(s+3.4)}\\
\frac{-0.06(s-0.5811)(s+6)}{(s+2)(s+3.4)}  
\end{array}\right]
\end{equation}
The robust stabilization problem can now be solved iff there a solution to the following optimization problem
\beq
\min_{Q\in M(\stabS)} \Vert T_{1}-T_{2}Q\Vert_{\infty}<1
\eeq

Converting this problem to Nehari problem which can be posed as for a given $R$ in $RL_{\infty}$ with dist $(R,\stabS)<1$, find all $X's$ in $\stabS$ such that $\Vert R-X \Vert_{\infty}\leq 1$ where $R=U_{i}^{*}T_{1}Y_{o}^{-1}$. Applying the steps in the algorithm from \cite{fran}, nearly optimal $Q$ can be computed. First, the inner-outer factorization of $T_{2}$ can be computed as $T_{2}=T_{2i}T_{2o}=U_{i}U_{0}$.
\begin{align}
U_{i}&=\left[\begin{array}{rr}
\frac{0.70711(s+1.242)(s-0.3131)}{(s+1.141)(s+0.4334)}\\
\frac{-0.70711(s-0.5811)(s+1)}{(s+1.141)(s+0.4334)}  
\end{array}\right]\\
U_{o}&=\frac{0.084853(s+0.4334)(s+1.141)(s+2)(s+3.4)(s+6)}{(s+1)(s+2)^{2}(s+3.4)^{2}}
\end{align}
As discussed in the \textbf{step 1} of the algorithm for solving the robust stabilization problem in matrix case, it is required to compute $RL_{\infty}$ matrix $Y$ which is given by, $Y=(I-U_{i}U_{i}^{*})T_{1}$.
\begin{equation}
Y=\left[\begin{array}{rr}
\frac{0.03(s+1)(s+0.5811)(s-1)(s+6)(s^{2}+4s+4.001)}{(s+1.141)(s-1.141)(s+0.4334)(s-0.4334)(s+2)(s+3.4)}\\
\frac{0.03(s+1)(s+6)(s+0.3131)(s-1.242)(s^{2}+4s+4.001)}{(s+1.141)(s-1.141)(s+0.4334)(s-0.4334)(s+2)(s+3.4)}  
\end{array}\right]   
\end{equation}

From above equation, $\Vert Y \Vert_{\infty}=0.3028$. Next, an upper bound $\gamma_{1}$ for $\gamma$ can be found which is $\gamma_{1}=\Vert T_{1} \Vert_{\infty}=1.5682$. Thus, $\beta$ lies in the interval ($\Vert Y \Vert_{\infty},\gamma_{1})=(0.3028,1.5682)$. For selecting a trial value for $\beta$ in this interval, binary search can be used. 

If $\beta > \Vert Y \Vert_{\infty}$, then the matrix $\beta^{2}-Y^{*}Y$ has a spectral factor $Y_{o}$ where $Y^{*}$ is complex conjugate transpose of the matrix $Y$. Let $R$ be $RL_{\infty}$ matrix defined as $R:=U_{i}^{*}T_{1}Y_{o}^{-1}$. $R$ depends on the value of $\beta$ selected. It is now required to find a closest matrix $X$ in $\stabS$ to a given matrix $R$ in $L_{\infty}$. The table \ref{table:1} below shows the variation of $\Vert\Gamma_{R}\Vert$ for different values of $\beta$.

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|}
\hline
$\beta$ & $\Vert\Gamma_{R}\Vert$ \\
\hline
0.9355 & 1.3004 \\
1.2518 & 0.9593 \\
1.0937 & 1.1035 \\
1.1728 & 1.0263 \\
1.2123 & 0.9916 \\
\hline
\end{tabular}
\caption{Table showing $\Vert\Gamma_{R}\Vert$ for various values of $\beta$ }
\label{table:1}
\end{table}

For each value of selected $\beta$, $R$ and $\Vert\Gamma_{R}\Vert$ is computed. For $\beta=1.2123, \Vert\Gamma_{R}\Vert=0.9916$ so this value of $\beta$ can be considered for which, ($\beta^{2}-Y^{*}Y$) has a spectral factor $Y_{o}$ which is as given below.
\begin{equation}
Y_{o}=\frac{1.2116(s+3.397)(s+1.14)(s+0.4208)}{(s+0.4334)(s+1.141)(s+3.4)}
\end{equation}
From the spectral factor $Y_{o}$, $R=U_{i}^{*}T_{1}Y_{o}^{-1}$ can be easily computed which is given by the following equation.
\begin{equation}
R=\frac{-0.03501(s+37.99)(s+6)(s+1.141)(s+1.139)(s+0.433)(s+0.4226)(s-1.101)}{(s-1.141)(s-0.4334)(s+1.14)(s+1)(s+2)(s+3.397)(s+0.4208)}
\end{equation}
Since $R$ is a scalar valued function, following theorem as found in \cite{fran} can be applied to find the closest function $X$ in $\stabS$.
\begin{theorem}
The infimal model matching error in model matching error equals  $\Vert \Gamma_{R} \Vert$, the unique optimal $X$ equals $R-\gamma (\frac{f}{g})$ and for the optimal $Q$, $T_{1}-T_{2}Q$ is all pass. 
\end{theorem}

The algorithm to compute $X$, when $R$ is scalar valued, can be found in \cite{fran}. It  is given below for reference and  applicable for this example.
\begin{enumerate}
\item [\textbf {Step 1}] Factor $R$ as $R=R_{1}+R_{2}$ where $R_{1}$ is strictly proper and analytic in Re s $\leq$ 0 while $R_{2}$ belongs to $\stabS$. $R_{1}$ has a minimal state space realization with $A,B,C$ as its matrices and matrix $A$ is antistable. 
\item [\textbf {Step 2}] Solve the following equations for $L_{c}$ and $L_{o}$.
\begin{align}
AL_{c}+L_{c}A^{T}&=BB^{T} \notag \\
A^{T}L_{o}+L_{o}A&=C^{T}C \notag
\end{align}
\item [\textbf {Step 3}] Find the maximum eigenvalue $\lambda^{2}$ of $L_{c}L_{o}$ and a corresponding eigenvector $w$. Defining $v:\lambda^{-1}L_{o}w$ so that from equation $L_{c}L_{o}w=\lambda^{2}w$, following pair of equations can be obtained. Solve the equation for $v$.
\begin{align*}
L_{c}v=\lambda w  \\
L_{o}w=\lambda v
\end{align*}
\item [\textbf {Step 4}] Define the real rational functions $f(s)$ and $g(s)$ as shown below.
\begin{align}
f(s)&:=
\left[\begin{array}{c|c}
A & w \\
\hline
C & 0
\end{array}\right]=C(sI-A)^{-1}w \notag \\
g(s)&:=
\left[\begin{array}{c|c}
-A^{T} & v \\
\hline
B^{T} & 0
\end{array}\right]=B^{T}[sI-(-A^{T})]^{-1}v \notag
\end{align}
\item [\textbf {Step 5}] Set the model matching error $\gamma=\lambda$ so that $X=R-\gamma (\frac{f}{g})$.
\item [\textbf {Step 6}] Solve for $Q$ in $\stabS$ using $X$ as obtained in \textbf{step 5}.    
\end{enumerate}

Using these steps from the algorithm, $X$ and hence $Q$ as a solution to the robust stabilization problem can be computed. From \textbf{step 1}, $R$ can be factored as $R=R_{1}+R_{2}$. $R_{1}$ and $R_{2}$ are respectively given by following equations.
\begin{align}
R_{1}&=\frac{-0.090464(s-1.09)}{(s-0.4334)(s-1.141)} \\
R_{2}&=\frac{-0.035018(s+1.14)(s+1.097)(s+0.4206)(s^{2}+19.11s+121)}{(s+0.4208)(s+1)(s+1.14)(s+2)(s+s+3.397)}
\end{align}
$R_{1}$ has a minimal state space realization with matrix $A$ antistable. The state space realization of $R_{1}$ is as given below.
\begin{align}
A&=\left[\begin{array}{rr}
0.4334 & 0.8104\\
0 & 1.1410 
\end{array}\right] \notag \\
B&= \left[\begin{array}{rr}
0 \\
1 
\end{array}\right]\notag \\
C&= \left[\begin{array}{rr}
0.7331 & -0.9046\\
\end{array}\right]\notag
\end{align}
The Lyaupnov equations given in \textbf{step 2} can be solved so as to obtain the controllability and observability grammians which are as given below.
\begin{align}
L_{c}&=\left[\begin{array}{rr}
0.4218 & -0.2256\\
-0.2256 & 0.4382 
\end{array}\right] \notag \\
L_{o}&= \left[\begin{array}{rr}
0.6201 & -0.7405\\
-0.7405 & 0.8846 
\end{array}\right]\notag 
\end{align}
The largest eigenvalue of $L_{c}L_{o}$ denoted as $\lambda^{2}$ is $0.9833$ and the corresponding eigenvector $w$ such that $L_{c}L_{o}w=\lambda^{2}w$ holds is as given below,
\begin{equation}
w= \left[\begin{array}{rr}
0.6782 \\
-0.7349 
\end{array}\right] \notag
\end{equation}
$v$ which is defined as $\lambda^{-1}L_{o}w$ can be computed by solving the equation $L_{o}w=\lambda v$ and is as given below.
\begin{equation}
v= \left[\begin{array}{rr}
0.9729 \\
-1.1620 
\end{array}\right] \notag
\end{equation}
The real rational functions $f(s)$ and $g(s)$ as defined in \textbf{step 4} can now be computed and are given below.
\begin{align}
f(s)&=\frac{1.162s-1.292}{s^{2}-1.574s+0.4945} \\
g(s)&=\frac{-1.162s-1.292}{s^{2}+1.574s+0.4945}
\end{align}
From \textbf{step 5}, the model matching error $\gamma=\lambda=\sqrt{0.9833}=0.9916$. Using this value of $\lambda$, $X$ can be obtained which is given below.
\begin{equation}
X=R-\gamma \Big(\frac{f}{g}\Big)=\frac{0.95658(s+4.27)(s+1.141)(s+1.141)(s+0.4331)}{(s+1.112)(s+1)(s+2)(s+3.397)}  
\end{equation}
Solving for $Q$ using the equation $X=U_{o}QY_{o}^{-1}$, it is possible obtain $Q$ which is given below.
\begin{equation}
Q=U_{o}^{-1}XY_{o}=\frac{13.6584(s+1.141)(s+0.4208)(s+4.27)}{(s+1.112)(s+6)(s+0.4334)}  
\end{equation}
The compensating network $Z_{c}$ can be expressed in terms of the free parameter $Q$ as below.
\begin{equation}
Z_{c}=\frac{Y+NQ}{X-DQ}  
\end{equation}
Using the expressions for $N,D,X,Y$ and $Q$ already computed, the compensating network $Z_{c}$ for the given network $Z$ can be computed which is given below.
\begin{equation}
\label{compnetwork}
Z_{c}=\frac{-1.0732(s+3.455)(s+1)}{(s+1.231)(s+3.387)}
\end{equation}
The compensating network $Z_{c}$ as given by equation (\ref{compnetwork}) ensures the robust stability of the interconnected network under $\pm 5\%$ variations in the parameters of the given network. 

\subsection{Results}
For this circuit example, it can now be shown that the impedance of the interconnected network $\tilde Z_{T}=(\tilde Z^{-1}+Z_{c}^{-1})^{-1}$ under parametric variations of $\pm 5\%$ is in $\stabS$. Consider the perturbed impedance $\tilde Z$ as given by equation (\ref{tildeimpedance}) with each parameter undergoing a variation of say,$+5\% $, as one of the possible variations. Now, it can be shown that the impedance of the interconnected network $\tilde Z_{T}$ is in $\stabS$.
\begin{align*}
\tilde Z_{T}&=(\tilde Z^{-1}+Z_{c}^{-1})^{-1} \notag \\
&=\Big\{\Big[\frac{1.05(s+0.9268)(s-0.5579)}{(s+1.171)(s-0.2951)}\Big]^{-1} + \Big[\frac{-1.0732(s+3.455)(s+1)}{(s+1.231)(s+3.387)}\Big]^{-1}\Big \}^{-1}\\
\therefore \ \tilde Z_{T}&=\frac{48.5413(s+3.455)(s+1)(s+0.9268)(s-0.5579)}{(s+16.24)(s+2.462)(s+1.462)(s+0.7239)}
\end{align*}
This shows that the perturbed impedance of the interconnected network $\tilde Z_{T}$ for one set of the parameter variations is in $\stabS$. 

\subsection{Discussion}
Perturbed impedance, $\tilde Z_{T}$ for one set of parameter variations is observed to be in $\stabS$. For other set of the parameter variations, $\tilde Z$ can similarly be computed and it can be shown that the perturbed impedance of the interconnected network $\tilde Z_{T}$ with the compensating network, $Z_{c}$ connected in parallel with $\tilde{Z}$ is also found to be in $\stabS$. The pole-zero plot for $\tilde Z_{T}$ for each set of parametric variations is as shown in the Fig.\ref{fig06a:name} and it can be seen that the all the poles of $\tilde Z_{T}$ lie in the left half plane.
\begin{figure}[h]
\centering
\includegraphics[width=15.0cm,height=10cm]{polezerozt}
\caption{Pole-zero plot of $\tilde Z_{T}$ for all parameter variations}\label{fig06a:name}
\end{figure}
Thus, the compensator $Z_{c}$ robustly stabilizes the given network under uncertainties and perturbations due to parameter variations.

\section{Conclusion}
\label{robustconsec} 
Robust stabilization problem in case of active multiport networks is formulated and solved in this chapter. Robustness is an important consideration in multiport interconnections as network undergoes perturbations and uncertainties due to parametric variations, model errors, disturbances and other parasitic effects which are inevitable. It may be possible that the the interconnected network is unable to meet the prescribed performance specifications or even become unstable if robustness is not considered during the design of a compensating network. The solution to robust stabilization problem can be obtained by approaches well known in modern system theory. An illustrative circuit example considered in this chapter shows that the compensating network obtained after solving the robust stabilization problem robustly stabilizes the given network under parametric variations. 
%%%%%%%%%%%%


